Topological Interpretations of GPT-3

This is an experiential study of investigating a consistent method for deriving the correlation between sentence vector and semantic meaning of a sentence. We first used three state-of-the-art word/sentence embedding methods including GPT-3, Word2Vec, and Sentence-BERT, to embed plain text sentence strings into high dimensional spaces. Then we compute the pairwise distance between any possible combination of two sentence vectors in an embedding space and map them into a matrix. Based on each distance matrix, we compute the correlation of distances of a sentence vector with respect to the other sentence vectors in an embedding space. Then we compute the correlation of each pair of the distance matrices. We observed correlations of the same sentence in different embedding spaces and correlations of different sentences in the same embedding space. These observations are consistent with our hypothesis and take us to the next stage.

==> tex/data.tex <==



==> tex/distancematrix.tex <==
To find the correlation between sentences in a cloud of word. A way is to construct matrices with varies distance and then find the correlations between those matrices. 

Several matrices we could use are listed below.
\subsection{Bottleneck Distance}
Briefly, the bottleneck distance is defined as 
$$ d_{\operatorname{B}} (\operatorname{D}(f), \operatorname{D}(g)) \leq \|f - g \|_{\infty}, $$ where $f$ and $g$ are two functions, and $\operatorname{D}(f)$ and $\operatorname{D}(g)$ are their corresponding persistence diagrams. The bottleneck distance stably bounds the latten distance.

\subsection{Adapted Levenshtein Distance}
The original levenshtein distance is a string metric for measuring the difference between two sequences in the alphabetic level\footnotemark{} \footnotetext{
The Levenshtein distance between two strings $x, y$ is denoted by $\operatorname{lev}(x, y)$ where
$$\operatorname{lev}(x, y) = \begin{cases}
  |x| & \text{ if } |y| = 0, \\
  |y| & \text{ if } |x| = 0, \\
  \operatorname{lev}\big(\operatorname{tail}(x),\operatorname{tail}(y)\big) & \text{ if } x[0] = y[0], \\
  1 + \min \begin{cases}
          \operatorname{lev}\big(\operatorname{tail}(x), y\big) \\
          \operatorname{lev}\big(x, \operatorname{tail}(y)\big) \\
          \operatorname{lev}\big(\operatorname{tail}(x), \operatorname{tail}(y)\big) \\
       \end{cases} & \text{ otherwise.}
\end{cases}
$$}. We have adapted it in the word level. Adapting it to the numeric type is the next thing to do. 




\section{Correlation Evaluation Methods}
Cross decomposition algorithms find the fundamental relations between two matrices. They are latent variable approaches to modeling the covariance structures in these two spaces. They will try to find the multidimensional direction in the $X$ space that explains the maximum multidimensional variance direction in the $Y$ space. In other words, PLS projects both $X$ and $Y$ into a lower-dimensional subspace such that the covariance between transformed $X$ and $Y$ is maximal.

\subsection{Canonical Correlation Analysis}
Canonical Correlation Analysis (CCA) is suited when the matrix of predictors has more variables than observations, and when there is multicollinearity among the features. By contrast, standard linear regression would fail in these case unless it is regularized. This estimator is unstable if the number of features or targets is greater than the number of samples. 

\subsection{Multi-dimensional Scaling}

Multidimensional scaling (MDS) is a low-dimensional representation of high-dimensional data in which the distances respect well the distances in the original high-dimensional space.

We could use MDS to analyze similarity or dissimilarity of two sentences, by modeling similarity or dissimilarity of two sentences embedded in a latent space as distances in a geometric space. 

Let $S$ be the similarity matrix, and $X$ the coordinates of the $n$ input points. Disparities $\hat{d_{ij}}$ are transformation of the similarities chosen in some optimal ways. The objective, called the stress, is then defined by $\sum_{i<j} d_{ij}(X) - \hat{d_{ij}}(X)$. 

There are two types of MDS algorithms: 
\subsubsection{Metric MDS} 
\hfill

The input similarity matrix arises from a metric. The distances between output two points are then set to be as close as possible to the similarity or dissimilarity data. 

Metric MDS called absolute MDS, disparities are defined by $\hat{d_{ij}} = S_{ij}$. With absolute MDS, the value $S_{ij}$ should then correspond exactly to the distance between point $i$ and $j$ in the embedding point. In general, disparities are set to $\hat{d_{ij}} = b S_{ij}$.

\subsubsection{Non-metric MDS} 
\hfill

The algorithms will try to preserve the order of the distances, and seek for a monotonic relationship between the distances in the embedded space and the similarities/dissimilarities.

Non metric MDS focuses on the ordination of the data. If $S_{ij} < S_{jk}$, then the embedding should enforce $d_{ij} < d_{jk}$. A simple algorithm to enforce that is to use a monotonic regression of $d_{ij}$ on $S_{ij}$, yielding disparities $\hat{d_{ij}}$ in the same order as $S_{ij}$.


==> tex/embedding.tex <==
\subsection{Sentence Embeddings}
\subsubsection{Doc2Vec\cite{le2014distributed} } 
\hfill

Doc2Vec is used to vectorize sentences using a similar approach as Word2Vec\cite{mikolov2013efficient}. Two word vectors that are close to each other have similar meanings. How about two sentence vectors are closed to each other? Do these two sentences have similar meanings? Two sentences could either have similar sentiment, or topic. What does the sentence vector represent for?

Finding the textual vector representations for machine to process the language is fundamental yet challenging in applications of natural language processing, due to the ambiguity presented in all levels of language \cite{sezerer2021survey}. In analogy with human's processing of texts, semantic clues, contextual and word knowledge are all required. Hence, two different computational systems are proposed for language processing, one is knowledge system, the other is the statistical system for vector representations.

{\bf One-hot encoding} of binary vector space is a simple technique among the method of statistical system. In each word vector, one-hot encoding uses the positional indices one to indicate the corresponding word, and zero elsewhere in the vector, which result in a three dimensional tensor representing the paragraphs. For a document including $N$ unique words, the last dimension of the tensor should be $N$. However, the drawback with this technique is for very large corpus and hence large $N$, the vector representation will be very sparse, which will lead to difficulties in computational processing. Moreover, one-hot encoding does capture the contextual and semantic information such as the similarity of two different words can not be compared. 

{\bf Bag of words} representation is another similar simple statistical model which focuses on multiplicity, which, however, disregard the order of the words and account for little semantic information. To tackle the issue present in one-hot encoding, the word vectors are introduced by Tomas Mikolov and etc \cite{mikolov2013efficient}. The neural network model \cite{mikolov2013efficient} proposed by Tomas Mikolov can learn high quality word vectors with relatively low computational costs. It is also found that learned vectors are able to capture the syntactic and semantic similarities. Inspired by the same idea of utilizing the unsupervised training, the method of paragraph vector is proposed to generate sentence level embedding. The method, in the next word prediction task, also uses the unique paragraph token as the feature input. The paragraph vector is able to outperform all other state-of-the-art models such as the word of vector averaging on classification and sentiment tasks. However, according to the result of our analysis, the model is yet to sufficiently capture the knowledge of syntactics. 

{\bf TF-IDF} is a common term weighting scheme in information retrieval, especially in text classification. It is defined as:

For each term $t$ in terms of all documents $d$, the weighted importance $w_{t,d}$ in all documents, 
$$ w_{t,d} = tf_{t,d} idf(w) = \frac{n_{t,d}}{ \sum_{t=1}^{k} n_{t,d} } log(\frac{N}{df(t)}),  $$ where $n_{t,d}$ means the total number of times that term $t$ appears in document $d$, this is computed in the last step, $\sum_{t=1}^{k} n_{t,d}$ is the total number of terms in the document, $N$ is the total number of documents, $df(t)$ is the number of documents that contain the term $t$. Documents in our case represents sentences. The goal of using TF-IDF is to scale down the impact of tokens that occur very frequently but empirically are less informative than features that occur less frequently.

\subsubsection{SentenceBERT, InferSent, Universal Sentence Encoder}
We will look into the other sentence embedding methods later.

\subsection{Word Embeddings}
\subsubsection{Word2Vec vs GPT-2 word embedding}

GPT-2 word embedding is context depending, however, Word2Vec word embedding does not depend on context\footnotemark{} \footnotetext{https://ai.stanford.edu/blog/contextual/}.



==> tex/othertda.tex <==

\section{An Introduction to a New Text Classification and Visualization for Natural Language Processing Using Topological Data Analysis \cite{DBLP:journals/corr/abs-1906-01726}}

This an empirical case study of using ``persistence homology'' and ``mapper'' to authorize each persian poem to either ``Ferdowsi'' or ``Hafez''. Authorship attribution is one of the text classification problem, which tries to identify the author of a given text based on its content. There are two main methods for authorship attribution problem: 
\begin{itemize}
    \item Non-Semantic - identify author based on the length of words/sentences and the vocabulary used in a given text; 
    \item Semantic - consider the structure of the language based its semantic analysis; 
    \item {\bf TDA} - a new state-of the-art method.
\end{itemize}
 A barcode represents each persistent generator(classes that generate p-th homology group) with a horizontal line beginning at the first filtration level where it appears, and ending at the filtration level where it disappears.
 A persistence diagram plots a point for each generator with its x-coordinate the birth time and its y-coordinate the death time. A visual representation of persistent homology is persistent diagram.
 
 Since it is very hard to analyze the information about homological groups and holes we can use a visualization method called “Barcode”, the idea is as follows: if a hole appears in $\theta_{t1}$ we start to draw a line where the beginning of the line is at $\theta_{t1}$ x-axis and if die in $\theta_{t2}$ e stop drawing the line and end of the line would be at $\theta_{t2}$.
%1) Any important definitions not covered in this course, e.g. a new type of complex/filtration used.
%2) If there are theoretical results, what are the important ones (usually denoted "Theorem")?  You don't need to state (or understand) any proofs.
%3) If there are empirical results, what are the key points?  What are the methods of the paper compared against?
%a) Do you think the results are reasonably reproducible?  Is there code or data provided?

\subsubsection{Compute Persistent Homology} % 3.2 P7
\hfill

\begin{itemize}
    \item First, they sketch presistent diagram, barcode and persistent landscapes for a sample of Ferdowsi poems including 1000 hemistich;
    \item Second, they divided 8000 hemistich of ``hafez'' to 8 parts with length 1000, then computed persistent diagram and first landscape of each part; 
    \item Third, they sketched the mean landscape of these parts;
    \item Finally, they computed Wasserstein distances between persistent Diagrams of correspondance parts of “hafez” and “Ferdowsi” poems.
\end{itemize}

\subsubsection{TDA Mapper in text classification}
\hfill

\begin{itemize}
    \item Gathering ans pre-processing the data of poems;
    \item Using TF-IDF algorithm to turn pre-processed data into a matrix which columns represent a single word in the entire corpus and each row represent  hemistich. The matrix is of the form $[9000*67671]$ (# hemistich *# words in corpus);
    \item Zoomed data $[100*100]$;
    \item Using truncated SVD and T-SNE algorithm as filter functions;
    \item Bining: the whole 2-dimensional space divided into smaller bins; 
    \item Clustering: clustering algorithms applied to each bin in order to create the nodes in the final graph;
    \item Output of the algorithm as a graph, every node in the graph is a cluster of the previous step and nodes share an edge if they have the data point in common.  
\end{itemize}

\section{Artificial Text Detection via Examining the Topology of Attention Maps\cite{DBLP:journals/corr/abs-2109-04825}}
This paper propose three novel types of interpretable topological features extracted from the attention graphs. This work empirically shows that the features derived from the BERT model outperform count-based and neural-based baselines up to 10\% on three common datasets, and tend to be the most robust towards unseen GPT-style generation models as opposed to existing methods. 

In this paper, the persistence features are considered as the numerical characteristic of the semantic evolution processes in the attention head.

\subsection{Topological Features} 
Topological Features include a set of graph properties, including the number of connected components, the number of edges, and the number of cycles. These features are calculated for each predefined threshold separately and then concatenated. They consider two following variants of the feature calculation: directed and un-directed attention graph. 

Topological features deal with clusters of mutual influence of the tokens in the sentence and the local structures like chains and cycles.

\subsubsection{Definition}
\hfill

First, fix a set of thresholds $T = \{t_i\}^k_{i=1}, 0<t_1<...<t_k<1$. 

Consider an attention head $h$ and corresponding weights $W^{attn} = (w^{attn}_{i,j}).$

Given a text sample $s$, for each threshold level $t\in T$ we define the weighted directed graph $\Gamma^h_s(t)$ with edges $\{j \rightarrow i | w^{attn}_{ij} \ge t\}$ and its undirected variant $\overline{\Gamma^h_s(t)}$ by setting an undirected edge $v_iv_j$ for each pair of vertices $v_i$ and $v_j$ which are connected by an edge in at least one direction in the graph $\Gamma^h_s(t)$. 

We consider the following features of the graphs: 
\begin{itemize}
    \item the first two Betti numbers of the undirected graph $\overline{\Gamma^h_s(t)}$. The feature calculation procedure is described in \ref{alg:1}.
    \item The number of edges $(e)$, the number of strongly connected components $(s)$ and the amount of simple directed cycles $(c)$ in the directed graph $\Gamma^h_s(t)$. 
\end{itemize}
To get the whole set of topological features for the given text sample $s$ and the attention head $h$, we concatenate the features for all the thresholds, starting from $T$.





\begin{algorithm}
\caption{Topological Features Calculation} \label{alg:1}
\begin{algorithmic}
\Require Text sample $s$
\Require Set of chosen attention heads $H_M$ of model $M$
\Require Thresholds array $T$
\Require Topological feature $f$ of unweighted graph
\Ensure Features array $Features$
\State {\bf procedure} \operatorname{FEATURES\_ CALC}($s$,  $H_M$, $T$)
    \State \hspace{0.3cm} {\bf for all } {h \in H_M, t\in T} {\bf do}
    
        \State \hspace{0.7cm} Calculate attention graph $\Gamma^h_s = (V, E, W^{att}_{h,s})$ on sample $s$ on head $h$
        \State \hspace{0.7cm} $E^h_s(t) \leftarrow \{e \in E(\Gamma^h_s) : W^{att}_{h,s} (e) \ge t \}$
        \State \hspace{0.7cm} $\Gamma^h_s(t) \leftarrow (V, E^h_s(t))$
        \State \hspace{0.7cm} $\overline{E^h_s(t)} \leftarrow \{ \{i, j\}:(i,j) \in E^h_s(t) \}$ 
        \State \hspace{0.7cm} $\overline{\Gamma^h_s(t)} \leftarrow (V,\overline{E^h_s(t)}) $ 
        \State \hspace{0.7cm} Calculate $f(\overline{\Gamma^h_s(t)})$    
    \State \hspace{0.3cm} {\bf end for }  
\State \hspace{0.3cm} $Features \leftarrow [ f(\overline{\Gamma^h_s(t)} ) ]^{h\in H_M}_{t\in T}$
\State \hspace{0.3cm} {\bf return } $Features$
\State {\bf end procedure}
\end{algorithmic}
\end{algorithm}




\subsection{Barcode Features} 
Barcode features are extracted from barcodes. 

The barcode features characterize the severity and robustness of the semantic changes. The features with long persistence - large distance between “birth” and “death” - correspond to the stable processes which dominate the others, while short segments in the barcode define processes highly influenced by noise.

For each text sample we calculate barcodes of the first two persistent homology groups (denoted as $H_0$ and $H_1$) on each attention head of the BERT model. We compute the following characteristics of these barcodes:
\begin{itemize}
    \item The sum of lengths of bars;
    \item The mean of lengths of bars;
    \item The variance of lengths of bars;
    \item The number of bars with time of birth/death greater/lower than threshold;
    \item The time of birth/death of the longest bar (excluding infinite);
    \item The overall number of bars;
    \item The entropy of the barcode.
\end{itemize}

\subsubsection{Persistent Homology and Betti Numbers}

 \hfill 
 
Recall that a simplicial complex $K$ is a collection of subsets of a finite set called $simplices$ such that each subset of any element of $K$ also is an element of $K$; such subsets of a simplex are called $faces$. In particular, an undirected graph is a simplicial complex where the simplices correspond to the edges and vertices of the graph. The set of all formal $\mathbb{Z}$-linear combinations of the $p$-dimensional simplices ($(p + 1)$-element finite sets from the collection) of $K$ is denoted $\mathsf{C}_p (K)$. These linear combinations $c =  \sum_j \gamma_j \sigma_j $ are called $p-chains$, where the $\gamma_j \in \mathbb{Z}$ and the $\sigma_j$ are $p$-simplices in $K$.

The boundary, $\partial(\sigma_j )$, is the formal sum of the $(p-1)$-dimensional faces of $\sigma_j$ and the boundary of the chain is obtained by extending $\partial$ linearly,
$$ \partial(c) = \sum_j \gamma_j \partial(\sigma_j)$$ for $c$ as above. 

The $p$-chains that have boundary 0 are called $p-cycles$, they form a subgroup $\mathsf{Z}_p(K)$ of $\mathsf{C}_p(K)$. The $p$-chains that are the boundary of $(p+1)$-chains are called $p$-boundaries and form a subgroup $\mathbf{B}_p(K)$ of $\mathsf{C}_p(K)$. The quotient group $\mathsf{H}_p(K) = \mathsf{C}_p(K)/\mathsf{B}_p(K)$ is called the $p$-th $homology$ of $K$. Their ranks $\beta_p = rk(\mathsf{H}_p(K))$ of these abelian groups are called $Betti$ $numbers$. The homology and the Betti numbers are classical topological invariants of $K$.


\subsection{Distance To Patterns} 
Distance to patterns is the group of features derived from the attention maps by computing the distance to the attention patterns. 

Pattern features provide a straightforward measure of the presence of typical processes over the whole sentence. The so-called “vertical” pattern corresponds to the “radiation” around the single token when the meaning of the sentence or a part of the sentence is aggregated from all words equally. “Diagonal” pattern represents consequent “concatenation” structure, going through all the sentence and thus reflecting the dependence of each token’s meaning on its left context.

They formalize these attention patterns and calculate the distances to them as follows.
Let $A = (a_{ij})$ be an incidence matrix of the graph $\Gamma$ with $n$ vertices, where $a_{ij} =1$ for all edges $(ij) \in E$ and $0$ for all other $i,j$. Let $\Gamma =(V,E)$ and $\Gamma' = (V,E')$ be two graphs with the same set of vertices, and let $A, A'$ be their incidence matrices. As a distance d between such graphs we use Frobenius norm of the difference $\|A - A'\|_F =
\sqrt{\sum_{i,j}(a_{ij} - a'_{ij})^2}$, normalized by the norms of the matrices of compared graphs:

$$ d(\Gamma, \Gamma') = \frac{\|A - A'\|_F}{\sqrt{\|A\|^2_F - \|A'\|^2_F}} = \sqrt{\frac{\sum_{i,j}(a_{ij}-a'_{ij})^2}{\sum_{i,j}(a_{ij}^2+a'_{ij}^2)}}.$$

Such distance takes values between 0 and 1. For the unweighted graphs we have: 

$$d(\Gamma, \Gamma') = \sqrt{\frac{|E\Delta E'|}{|E|+|E'|}}, $$ where $E \Delta E' = (E / E') \bigcup (E'/ E) $ is the symmetric difference of sets $E$ and $E'$. 

We consider distances from the given graph $\Gamma$ to attention patterns $\Gamma_i$ as the graph features $d_i(\Gamma) = d(\Gamma,\Gamma_i)$, and the patterns posed by
\begin{itemize}
    \item Attention to the previous token. $\Gamma_{feature}$ : $E = (i + 1, i), i = \overline{1, n-1}$.
    \item Attention to the next token. $\Gamma_{feature}$ :$ E = (i, i + 1), i = \overline{1, n-1}$.
    \item Attention to $[CLS]$-token. $[CLS]$-token corresponds to the vertex 1 of the set $V = [1,n]$ as it denotes the beginning of the text. $\Gamma_{feature}$ : $E = (i, 1), i = \overline{1, n}$.
    \item Attention to $[SEP]$-token. Suppose $i_1, . . . , i_k$ are the indices of $[SEP]$-tokens. Then $\Gamma_{feature}$ : $E = (i, i_t), i = \overline{1, n}, t = \overline{1, k}$.
    \item Attention to punctuation marks. Let $i_1,...,i_k$ be the indices of the tokens which correspond to commas and periods. $\Gamma_{feature}$ : $E =
(i,i_t), i = \overline{1,n}, t = \overline{1,k}$. Note that this pattern can be potentially divided into Attention to commas and Attention to periods.

\end{itemize}

\section{RipsNet\cite{DBLP:journals/corr/abs-2202-01725}}

The applications of topological descriptors, such as, PDs, have two limitations, one is computational complexity required to exactly compute such descriptors, and the other is the sensitivity to even low-level proportions of outliers. This work propose to bypass these two burdens in a data-driven setting, RipsNet, by entrusting the estimation of PDs built on top of point clouds to a neural network architecture. The advantages of RipsNet are
\begin{itemize}
    \item Once trained on a given data set, RipsNet can estimate topological descriptors on test data very efficiently with generalization capacity.
    \item Furthermore, they proved that RipsNet is robust to input perturbations in terms of the 1-Wasserstein distance, a major improvement over the standard computation of PDs that only enjoys Hausdorff stability, yielding RipsNet to substantially outperform exactly-computed PDs in noisy settings. 
\end{itemize}
The contributions of this work are
\begin{itemize}
    \item Introduced RipsNet, a DeepSets-like architecture capable of learning finite-dimensional embeddings of Rips PDs built on top of point clouds. 
    \item They study the robustness properties of RipsNet. In particular, we prove that for a given point cloud X, perturbing a proportion $\lambda \in (0, 1)$ of its points can only change the output quantity even in the regime $\lambda \rightarrow 0$.
    \item They experimentally showcase how RipsNet can be trained to produce fast, accurate, and useful estimations of topological descriptors. They observe that using RipsNet outputs instead of exact PDs yields better performances for classification tasks based on topological properties.
\end{itemize}

RipsNet compute features that look like rips features, but does not helpful for any other interpretations. 
\subsubsection{Further reading - DeepSets\cite{DBLP:journals/corr/ZaheerKRPSS17}}

